Is it Time to Swish? Comparing Deep Learning Activation Functions Across NLP tasks

Activation functions play a crucial role in neural networks because they are the nonlinearities which have been attributed to the success story of deep learning. One of the currently most popular activation functions is ReLU, but several competitors have recently been proposed or 'discovered', including LReLU functions and swish. While most works compare newly proposed activation functions on few tasks (usually from image classification) and against few competitors (usually ReLU), we perform the first large-scale comparison of 21 activation functions across eight different NLP tasks. We find that a largely unknown activation function performs most stably across all tasks, the so-called penalized tanh function. We also show that it can successfully replace the sigmoid and tanh gates in LSTM cells, leading to a 2 percentage point (pp) improvement over the standard choices on a challenging NLP task.

==> plots/doc2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(8502.00,6802.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(784,1687){\makebox(0,0)[r]{\strut{} 79}}%
      \csname LTb\endcsname%
      \put(784,1960){\makebox(0,0)[r]{\strut{} 79.2}}%
      \csname LTb\endcsname%
      \put(784,2234){\makebox(0,0)[r]{\strut{} 79.4}}%
      \csname LTb\endcsname%
      \put(784,2507){\makebox(0,0)[r]{\strut{} 79.6}}%
      \csname LTb\endcsname%
      \put(784,2781){\makebox(0,0)[r]{\strut{} 79.8}}%
      \csname LTb\endcsname%
      \put(784,3054){\makebox(0,0)[r]{\strut{} 80}}%
      \csname LTb\endcsname%
      \put(784,3328){\makebox(0,0)[r]{\strut{} 80.2}}%
      \csname LTb\endcsname%
      \put(784,3601){\makebox(0,0)[r]{\strut{} 80.4}}%
      \csname LTb\endcsname%
      \put(784,3875){\makebox(0,0)[r]{\strut{} 80.6}}%
      \csname LTb\endcsname%
      \put(784,4148){\makebox(0,0)[r]{\strut{} 80.8}}%
      \csname LTb\endcsname%
      \put(784,4421){\makebox(0,0)[r]{\strut{} 81}}%
      \csname LTb\endcsname%
      \put(784,4695){\makebox(0,0)[r]{\strut{} 81.2}}%
      \csname LTb\endcsname%
      \put(784,4968){\makebox(0,0)[r]{\strut{} 81.4}}%
      \csname LTb\endcsname%
      \put(784,5242){\makebox(0,0)[r]{\strut{} 81.6}}%
      \csname LTb\endcsname%
      \put(784,5515){\makebox(0,0)[r]{\strut{} 81.8}}%
      \csname LTb\endcsname%
      \put(784,5789){\makebox(0,0)[r]{\strut{} 82}}%
      \csname LTb\endcsname%
      \put(784,6062){\makebox(0,0)[r]{\strut{} 82.2}}%
      \csname LTb\endcsname%
      \put(784,6336){\makebox(0,0)[r]{\strut{} 82.4}}%
      \csname LTb\endcsname%
      \put(784,6609){\makebox(0,0)[r]{\strut{} 82.6}}%
      \csname LTb\endcsname%
      \put(880,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}elu}}}%
      \csname LTb\endcsname%
      \put(1223,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}selu}}}%
      \csname LTb\endcsname%
      \put(1565,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}tanh}}}%
      \csname LTb\endcsname%
      \put(1908,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}minsin}}}%
      \csname LTb\endcsname%
      \put(2251,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-2}}}%
      \csname LTb\endcsname%
      \put(2593,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}penalized\_tanh}}}%
      \csname LTb\endcsname%
      \put(2936,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-3}}}%
      \csname LTb\endcsname%
      \put(3279,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}sin}}}%
      \csname LTb\endcsname%
      \put(3621,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-4}}}%
      \csname LTb\endcsname%
      \put(3964,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}prelu}}}%
      \csname LTb\endcsname%
      \put(4307,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}leakyrelu-0.3}}}%
      \csname LTb\endcsname%
      \put(4649,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}linear}}}%
      \csname LTb\endcsname%
      \put(4992,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxtanh}}}%
      \csname LTb\endcsname%
      \put(5334,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}leakyrelu-0.01}}}%
      \csname LTb\endcsname%
      \put(5677,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}relu}}}%
      \csname LTb\endcsname%
      \put(6020,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}tanhrev}}}%
      \csname LTb\endcsname%
      \put(6362,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}swish}}}%
      \csname LTb\endcsname%
      \put(6705,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}cosper}}}%
      \csname LTb\endcsname%
      \put(7048,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}sigmoid}}}%
      \csname LTb\endcsname%
      \put(7390,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxsig}}}%
      \csname LTb\endcsname%
      \put(7733,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}cube}}}%
      \put(7829,2171){\makebox(0,0)[l]{\strut{} 45}}%
      \put(7829,3059){\makebox(0,0)[l]{\strut{} 50}}%
      \put(7829,3946){\makebox(0,0)[l]{\strut{} 55}}%
      \put(7829,4834){\makebox(0,0)[l]{\strut{} 60}}%
      \put(7829,5721){\makebox(0,0)[l]{\strut{} 65}}%
      \put(7829,6609){\makebox(0,0)[l]{\strut{} 70}}%
      \csname LTb\endcsname%
      \put(128,4056){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6998,1807){\makebox(0,0)[r]{\strut{}Best}}%
      \csname LTb\endcsname%
      \put(6998,1647){\makebox(0,0)[r]{\strut{}Avg}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/doc2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/sent2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(8502.00,6802.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(784,1711){\makebox(0,0)[r]{\strut{} 75.2}}%
      \put(784,2156){\makebox(0,0)[r]{\strut{} 75.3}}%
      \put(784,2602){\makebox(0,0)[r]{\strut{} 75.4}}%
      \put(784,3047){\makebox(0,0)[r]{\strut{} 75.5}}%
      \put(784,3492){\makebox(0,0)[r]{\strut{} 75.6}}%
      \put(784,3937){\makebox(0,0)[r]{\strut{} 75.7}}%
      \put(784,4383){\makebox(0,0)[r]{\strut{} 75.8}}%
      \put(784,4828){\makebox(0,0)[r]{\strut{} 75.9}}%
      \put(784,5273){\makebox(0,0)[r]{\strut{} 76}}%
      \put(784,5718){\makebox(0,0)[r]{\strut{} 76.1}}%
      \put(784,6164){\makebox(0,0)[r]{\strut{} 76.2}}%
      \put(784,6609){\makebox(0,0)[r]{\strut{} 76.3}}%
      \put(880,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}relu}}}%
      \put(1223,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-4}}}%
      \put(1565,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}leakyrelu-0.01}}}%
      \put(1908,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-3}}}%
      \put(2251,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}penalized\_tanh}}}%
      \put(2593,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-2}}}%
      \put(2936,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}prelu}}}%
      \put(3279,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}minsin}}}%
      \put(3621,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}swish}}}%
      \put(3964,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}tanh}}}%
      \put(4307,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}selu}}}%
      \put(4649,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}sin}}}%
      \put(4992,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}leakyrelu-0.3}}}%
      \put(5334,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxtanh}}}%
      \put(5677,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxsig}}}%
      \put(6020,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}sigmoid}}}%
      \put(6362,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}cosper}}}%
      \put(6705,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}tanhrev}}}%
      \put(7048,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}cube}}}%
      \put(7390,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}elu}}}%
      \put(7733,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}linear}}}%
      \put(7829,2261){\makebox(0,0)[l]{\strut{} 50}}%
      \put(7829,3348){\makebox(0,0)[l]{\strut{} 55}}%
      \put(7829,4435){\makebox(0,0)[l]{\strut{} 60}}%
      \put(7829,5522){\makebox(0,0)[l]{\strut{} 65}}%
      \put(7829,6609){\makebox(0,0)[l]{\strut{} 70}}%
      \put(128,4056){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6998,6466){\makebox(0,0)[r]{\strut{}Best}}%
      \csname LTb\endcsname%
      \put(6998,6306){\makebox(0,0)[r]{\strut{}Avg}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/sent2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/sent3.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(8502.00,6802.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(784,1711){\makebox(0,0)[r]{\strut{} 75.2}}%
      \csname LTb\endcsname%
      \put(784,2156){\makebox(0,0)[r]{\strut{} 75.3}}%
      \csname LTb\endcsname%
      \put(784,2602){\makebox(0,0)[r]{\strut{} 75.4}}%
      \csname LTb\endcsname%
      \put(784,3047){\makebox(0,0)[r]{\strut{} 75.5}}%
      \csname LTb\endcsname%
      \put(784,3492){\makebox(0,0)[r]{\strut{} 75.6}}%
      \csname LTb\endcsname%
      \put(784,3937){\makebox(0,0)[r]{\strut{} 75.7}}%
      \csname LTb\endcsname%
      \put(784,4383){\makebox(0,0)[r]{\strut{} 75.8}}%
      \csname LTb\endcsname%
      \put(784,4828){\makebox(0,0)[r]{\strut{} 75.9}}%
      \csname LTb\endcsname%
      \put(784,5273){\makebox(0,0)[r]{\strut{} 76}}%
      \csname LTb\endcsname%
      \put(784,5718){\makebox(0,0)[r]{\strut{} 76.1}}%
      \csname LTb\endcsname%
      \put(784,6164){\makebox(0,0)[r]{\strut{} 76.2}}%
      \csname LTb\endcsname%
      \put(784,6609){\makebox(0,0)[r]{\strut{} 76.3}}%
      \csname LTb\endcsname%
      \put(880,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\relu}}}%
      \csname LTb\endcsname%
      \put(1223,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-4}}}%
      \csname LTb\endcsname%
      \put(1565,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}leakyrelu-0.01}}}%
      \csname LTb\endcsname%
      \put(1908,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-3}}}%
      \csname LTb\endcsname%
      \put(2251,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\pentan}}}%
      \csname LTb\endcsname%
      \put(2593,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxout-2}}}%
      \csname LTb\endcsname%
      \put(2936,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\prelu}}}%
      \csname LTb\endcsname%
      \put(3279,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\minsin}}}%
      \csname LTb\endcsname%
      \put(3621,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\swish}}}%
      \csname LTb\endcsname%
      \put(3964,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\mytanh}}}%
      \csname LTb\endcsname%
      \put(4307,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\selu}}}%
      \csname LTb\endcsname%
      \put(4649,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\mysin}}}%
      \csname LTb\endcsname%
      \put(4992,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}leakyrelu-0.3}}}%
      \csname LTb\endcsname%
      \put(5334,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\maxtanh}}}%
      \csname LTb\endcsname%
      \put(5677,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\maxsig}}}%
      \csname LTb\endcsname%
      \put(6020,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\sigmoid}}}%
      \csname LTb\endcsname%
      \put(6362,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\cosid}}}%
      \csname LTb\endcsname%
      \put(6705,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\arctid}}}%
      \csname LTb\endcsname%
      \put(7048,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\cube}}}%
      \csname LTb\endcsname%
      \put(7390,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\elu}}}%
      \csname LTb\endcsname%
      \put(7733,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}\linear}}}%
      \put(7829,2261){\makebox(0,0)[l]{\strut{} 50}}%
      \put(7829,3348){\makebox(0,0)[l]{\strut{} 55}}%
      \put(7829,4435){\makebox(0,0)[l]{\strut{} 60}}%
      \put(7829,5522){\makebox(0,0)[l]{\strut{} 65}}%
      \put(7829,6609){\makebox(0,0)[l]{\strut{} 70}}%
      \put(128,4056){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6998,6466){\makebox(0,0)[r]{\strut{}Best}}%
      \csname LTb\endcsname%
      \put(6998,6306){\makebox(0,0)[r]{\strut{}Avg}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/sent3}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> plots/seq2.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
  \setlength{\unitlength}{0.0500bp}%
  \begin{picture}(8502.00,6802.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%
      \put(592,2139){\makebox(0,0)[r]{\strut{} 51}}%
      \csname LTb\endcsname%
      \put(592,3256){\makebox(0,0)[r]{\strut{} 54}}%
      \csname LTb\endcsname%
      \put(592,4374){\makebox(0,0)[r]{\strut{} 57}}%
      \csname LTb\endcsname%
      \put(592,5491){\makebox(0,0)[r]{\strut{} 60}}%
      \csname LTb\endcsname%
      \put(592,6609){\makebox(0,0)[r]{\strut{} 63}}%
      \csname LTb\endcsname%
      \put(688,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}lrelu001}}}%
      \csname LTb\endcsname%
      \put(1158,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}relu}}}%
      \csname LTb\endcsname%
      \put(1627,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}swish}}}%
      \csname LTb\endcsname%
      \put(2097,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}penalized\_tanh}}}%
      \csname LTb\endcsname%
      \put(2567,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}lrelu030}}}%
      \csname LTb\endcsname%
      \put(3036,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}tanhrev}}}%
      \csname LTb\endcsname%
      \put(3506,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}elu}}}%
      \csname LTb\endcsname%
      \put(3976,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}minsin}}}%
      \csname LTb\endcsname%
      \put(4445,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxtanh}}}%
      \csname LTb\endcsname%
      \put(4915,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}tanh}}}%
      \csname LTb\endcsname%
      \put(5385,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}sin}}}%
      \csname LTb\endcsname%
      \put(5854,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}maxsig}}}%
      \csname LTb\endcsname%
      \put(6324,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}selu}}}%
      \csname LTb\endcsname%
      \put(6794,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}linear}}}%
      \csname LTb\endcsname%
      \put(7263,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}sigmoid}}}%
      \csname LTb\endcsname%
      \put(7733,1408){\rotatebox{-270}{\makebox(0,0)[r]{\strut{}cosper}}}%
      \put(7829,2818){\makebox(0,0)[l]{\strut{} 18}}%
      \put(7829,3679){\makebox(0,0)[l]{\strut{} 23}}%
      \put(7829,4541){\makebox(0,0)[l]{\strut{} 28}}%
      \put(7829,5403){\makebox(0,0)[l]{\strut{} 33}}%
      \put(7829,6264){\makebox(0,0)[l]{\strut{} 38}}%
      \put(128,4056){\rotatebox{-270}{\makebox(0,0){\strut{}Score}}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%
      \put(6998,6466){\makebox(0,0)[r]{\strut{}Best}}%
      \csname LTb\endcsname%
      \put(6998,6306){\makebox(0,0)[r]{\strut{}Avg}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{plots/seq2}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> problems.tex <==
\subsection{Size matters}
People compare sentence embeddings of different sizes, but at the same time state that the evaluation measure, log.reg., performs better with higher-dimensional inputs.

\textbf{TODO}: evaluate 100,200,...,2000 dimensional word2vec embeddings.

\subsection{Comparing the uncomparable}
Citing numbers from previous papers which evaluated differently makes no sense.

\textbf{TODO}: Give numbers from sent2vec paper and our own evaluation of the method \todo{AR: we could even compare senteval, our own framework, and their values.}

\subsection{Which Classifier to use?}
Most researchers feed in to log.reg., some others feed sentence embeddings to deep averaging networks and CNNs (google paper). This makes things very uncomparable. The questions that arises is among others: is log.reg.\ eval justified when the embeddings would subsequently be used with more powerful networks anyway?

\textbf{TODO}: eval google embeddings in our own framework and perform some correlation analyses between log.reg.\ and CNN or deep average networks.

\todo{AR: Maybe even: Evaluate infersent with deep network, our own method with deep network. compare. We can also show how the effect is xling. do we get a bigger drop then with deep averaging, CNN? not suitable in many scenarios then.}

\subsection{Using cosine and Pearson correlation for evaluation of embeddings}
Problems: cosine and Pearson are arbitrary choices. Cosine/Pearson are not robust against certain normalizations. These kinds of evaluations may therefore be misleading. Better: learn the embedding function. Moreover: the google guys propose a variant of cosine because it ``performed better'' \todo{We need to propose solutions for being accepted. Learning sim could be one of them.}

\textbf{TODO}: make an experiment with learned embedding function vs.\ cosine and the cosine variant suggested in the google paper. Use concatenated p-means as an illustration.

\subsection{Several simple sentence embeddings techniques perform quite badly}
They even underperform word2vec\todo{Glove trained on huge huge corpus, not word2vec} embeddings. Problems: sent2vec, SIF, Siamese CBOW were all either evaluated for cosine or compared to very bad, and arbitrary, reference points (sent2vec). \todo{AR: Well, some methods might serve a purpose: retrieval. but I show that sent2vec for example is crap in retrieval. SIF might be better.}

\subsection{Using GPU vs.\ CPU}
Well, that's a minor point \todo{AR: This is mostly comparing liblinear against pytorch logreg implementation. Not GPU vs CPU actually. So it depends on how you implement logreg, actually.}

\subsection{The universal tasks are not universal}
For some the majority baseline is quite high. They're all on sentiment. \todo{AR: Yeah, but there is also this COCO retrieval stuff and semantic similarity we ignored due to weird evaluation}

\subsection{Hyper-Parameter tuning of log.reg.}
Optimizing learning rate may be crucial? \todo{AR: I would rather say: if you dont do hyperparam optimization properly you will get results that are worse than with proper hyperparams PER EMBEDDING TYPE.}

\subsection{Embeddings are trained on different data}
But people make claims about the techniques (glove better than word2vec), which is something to keep in mind. \todo{AR: Yes its all about the training data. Similar to NMT. But people already know this I guess?}


